Frequency Dynamic Convolutions for Sound Event Detection

Recent research in deep learning-based Sound Event Detection (SED) has primarily focused on Convolutional Recurrent Neural Networks (CRNNs) and Transformer models. However, conventional 2D convolution-based models assume shift invariance along both the temporal and frequency axes, leadin to inconsistencies when dealing with frequency-dependent characteristics of acoustic signals. To address this issue, this study proposes Frequency Dynamic Convolution (FDY conv), which dynamically adjusts convolutional kernels based on the frequency composition of the input signal to enhance SED performance. FDY conv constructs an optimal frequency response by adaptively weighting multiple basis kernels based on frequency-specific attention weights. Experimental results show that applying FDY conv to CRNNs improves performance on the DESED dataset by 7.56% compared to the baseline CRNN. However, FDY conv has limitations in that it combines basis kernels of the same shape across all frequencies, restricting its ability to capture diverse frequency-specific characteristics. Additionally, the $3\times3$ basis kernel size is insufficient to capture a broader frequency range. To overcome these limitations, this study introduces an extended family of FDY conv models. Dilated FDY conv (DFD conv) applies convolutional kernels with various dilation rates to expand the receptive field along the frequency axis and enhance frequency-specific feature representation. Experimental results show that DFD conv improves performance by 9.27% over the baseline. Partial FDY conv (PFD conv) addresses the high computational cost of FDY conv, which results from performing all convolution operations with dynamic kernels. Since FDY conv may introduce unnecessary adaptivity for quasi-stationary sound events, PFD conv integrates standard 2D convolutions with frequency-adaptive kernels to reduce computational complexity while maintaining performance. Experimental results demonstrate that PFD conv improves performance by 7.80% over the baseline while reducing the number of parameters by 54.4% compared to FDY conv. Multi-Dilated FDY conv (MDFD conv) extends DFD conv by addressing its structural limitation of applying the same dilation across all frequencies. By utilizing multiple convolutional kernels with different dilation rates, MDFD conv effectively captures diverse frequency-dependent patterns. Experimental results indicate that MDFD conv achieves the highest performance, improving the baseline CRNN performance by 10.98%. Furthermore, standard FDY conv employs Temporal Average Pooling, which assigns equal weight to all frames along the time axis, limiting its ability to effectively capture transient events. To overcome this, this study proposes TAP-FDY conv (TFD conv), which integrates Temporal Attention Pooling (TA) that focuses on salient features, Velocity Attention Pooling (VA) that emphasizes transient characteristics, and Average Pooling (AP) that captures stationary properties. TAP-FDY conv achieves the same performance as MDFD conv but reduces the number of parameters by approximately 30.01% (12.703M vs. 18.157M), achieving equivalent accuracy with lower computational complexity. Class-wise performance analysis reveals that FDY conv improves detection of non-stationary events, DFD conv is particularly effective for events with broad spectral features, and PFD conv enhances the detection of quasi-stationary events. Additionally, TFD conv (TFD-CRNN) demonstrates strong performance in detecting transient events. In the case studies, PFD conv effectively captures stable signal patterns in tank powertrain fault recognition, DFD conv recognizes wide harmonic spectral patterns on speed-varying motor fault recognition, while TFD conv outperforms other models in detecting transient signals in offshore arc detection. These results suggest that frequency-adaptive convolutions and their extended variants provide a robust alternative to conventional 2D convolutions in deep learning-based audio processing.

==> department_names.tex <==
\newcommand{\department}[3]{%
    \ifthenelse{\equal{#1}{PH}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{물리학과}
        \renewcommand{\@childDeptNameEng}{Department of Physics}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Physics}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{MAS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{수리과학과}
        \renewcommand{\@childDeptNameEng}{Department of Mathematical Sciences}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Mathematical Sciences}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{CH}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{화학과}
        \renewcommand{\@childDeptNameEng}{Department of Chemistry}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Chemistry}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{NST}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{나노과학기술대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Nanoscience and Technology}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Nanoscience and Technology}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{QU}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{양자대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Quantum Science and Technology}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Quantum Science and Technology}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{BS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{생명과학과}
        \renewcommand{\@childDeptNameEng}{Department of Biological Sciences}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Biological Sciences}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{MSE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{의과학대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Medical Science and Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Medical Science and Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{BCS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{뇌인지과학과}
        \renewcommand{\@childDeptNameEng}{Department of Brain and Cognitive Sciences}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Brain and Cognitive Sciences}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{EB}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{공학생물학대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Engineering Biology}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Engineering Biology}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{SR}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{줄기세포및재생생물학대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Stem Cell and Regenerative Biology}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Stem Cell and Regenerative Biology}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{CE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{건설및환경공학과}
        \renewcommand{\@childDeptNameEng}{Department of Civil and Environmental Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Civil and Environmental Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{ME}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{기계공학과}
        \renewcommand{\@childDeptNameEng}{Department of Mechanical Engineering}
        \renewcommand{\@parentDeptNameKor}{기계항공공학부}
        \renewcommand{\@parentDeptNameEng}{School of Mechanical and Aerospace Engineering}
        \renewcommand{\@parentAcademNameEng}{Mechanical and Aerospace Engineering}
        \renewcommand{\@childAcademNameEng}{Mechanical Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{OSE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{해양시스템대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Ocean Systems Engineering}
        \renewcommand{\@parentDeptNameKor}{기계항공공학부}
        \renewcommand{\@parentDeptNameEng}{School of Mechanical and Aerospace Engineering}
        \renewcommand{\@parentAcademNameEng}{Mechanical and Aerospace Engineering}
        \renewcommand{\@childAcademNameEng}{Ocean Systems Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{AE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{항공우주공학과}
        \renewcommand{\@childDeptNameEng}{Department of Aerospace Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Aerospace Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{BIS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{바이오및뇌공학과}
        \renewcommand{\@childDeptNameEng}{Department of Bio and Brain Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Bio and Brain Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{BCE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{뇌인지공학프로그램}
        \renewcommand{\@childDeptNameEng}{Program of Brain and Cognitive Engineering}
        \renewcommand{\@parentDeptNameKor}{바이오및뇌공학과}
        \renewcommand{\@parentDeptNameEng}{Department of Bio and Brain Engineering}
        \renewcommand{\@parentAcademNameEng}{Bio and Brain Engineering}
        \renewcommand{\@childAcademNameEng}{Brain and Cognitive Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{ID}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{산업디자인학과}
        \renewcommand{\@childDeptNameEng}{Department of Industrial Design}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Industrial Design}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{CBE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{생명화학공학과}
        \renewcommand{\@childDeptNameEng}{Department of Chemical and Biomolecular Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Chemical and Biomolecular Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{MS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{신소재공학과}
        \renewcommand{\@childDeptNameEng}{Department of Materials Science and Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Materials Science and Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{EE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{전기및전자공학부}
        \renewcommand{\@childDeptNameEng}{School of Electrical Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Electrical Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{GSST}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{반도체공학대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Semiconductor Technology}
        \renewcommand{\@parentDeptNameKor}{전기및전자공학부}
        \renewcommand{\@parentDeptNameEng}{School of Electrical Engineering}
        \renewcommand{\@parentAcademNameEng}{Electrical Engineering}
        \renewcommand{\@childAcademNameEng}{Semiconductor Technology}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{AIS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{인공지능반도체대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of AI Semiconductor}
        \renewcommand{\@parentDeptNameKor}{전기및전자공학부}
        \renewcommand{\@parentDeptNameEng}{School of Electrical Engineering}
        \renewcommand{\@parentAcademNameEng}{Electrical Engineering}
        \renewcommand{\@childAcademNameEng}{AI Semiconductor}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{SSE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{반도체시스템공학과}
        \renewcommand{\@childDeptNameEng}{Department of Semiconductor System Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Semiconductor System Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{CS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{전산학부}
        \renewcommand{\@childDeptNameEng}{School of Computing}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Computing}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{IS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{정보보호대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Information Security}
        \renewcommand{\@parentDeptNameKor}{전산학부}
        \renewcommand{\@parentDeptNameEng}{School of Computing}
        \renewcommand{\@parentAcademNameEng}{Computing}
        \renewcommand{\@childAcademNameEng}{Information Security}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{SEP}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{소프트웨어대학원프로그램}
        \renewcommand{\@childDeptNameEng}{Software Graduate Program}
        \renewcommand{\@parentDeptNameKor}{전산학부}
        \renewcommand{\@parentDeptNameEng}{School of Computing}
        \renewcommand{\@parentAcademNameEng}{Computing}
        \renewcommand{\@childAcademNameEng}{Software}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{ICE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{정보통신공학과}
        \renewcommand{\@childDeptNameEng}{Department of Information and Communications Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Information and Communications Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{DMP}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{디지털미디어프로그램}
        \renewcommand{\@childDeptNameEng}{Digital Media Program }
        \renewcommand{\@parentDeptNameKor}{정보통신공학과}
        \renewcommand{\@parentDeptNameEng}{Department of Information and Communications Engineering}
        \renewcommand{\@parentAcademNameEng}{Information and Communications Engineering}
        \renewcommand{\@childAcademNameEng}{Digital Media}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{IE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{산업 및 시스템 공학과}
        \renewcommand{\@childDeptNameEng}{Department of Industrial and Systems Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Industrial and Systems Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{DS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{데이터사이언스대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Data Science}
        \renewcommand{\@parentDeptNameKor}{산업 및 시스템 공학과}
        \renewcommand{\@parentDeptNameEng}{Department of Industrial and Systems Engineering}
        \renewcommand{\@parentAcademNameEng}{Industrial and Systems Engineering}
        \renewcommand{\@childAcademNameEng}{Data Science}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{NQE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{원자력 및 양자공학과}
        \renewcommand{\@childDeptNameEng}{Department of Nuclear and Quantum Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Nuclear and Quantum Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{MO}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{조천식모빌리티대학원}
        \renewcommand{\@childDeptNameEng}{Cho Chun Shik Graduate School of Mobility}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Mobility}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{AI}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{김재철AI대학원}
        \renewcommand{\@childDeptNameEng}{Kim Jaechul Graduate School of AI}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{AI}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{PSE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{고분자학 학제전공}
        \renewcommand{\@childDeptNameEng}{Polymer Science and Engineering Program}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Polymer Science and Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{SPE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{우주탐사공학 학제전공}
        \renewcommand{\@childDeptNameEng}{Space Exploration Engineering Program}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Space Exploration Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{ENV}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{환경・에너지공학 학제전공}
        \renewcommand{\@childDeptNameEng}{Environmental and Energy Technology Program}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Environmental and Energy Technology}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{RE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{로봇공학 학제전공}
        \renewcommand{\@childDeptNameEng}{Robotics Program}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Robotics}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{PD}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{미래자동차 학제전공}
        \renewcommand{\@childDeptNameEng}{Division of Future Vehicle}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Future Vehicle}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{STE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{반도체 학제전공}
        \renewcommand{\@childDeptNameEng}{Semiconductor Technology Educational Program}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Semiconductor Technology}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{TE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{정보통신공학 학제전공}
        \renewcommand{\@childDeptNameEng}{Telecommunication Engineering Program}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Telecommunication Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{GGS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{녹색성장지속가능대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Green Growth and Sustainability}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Green Growth and Sustainability}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{MV}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{메타버스대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Metaverse}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Metaverse}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{HSS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{디지털인문사회과학부}
        \renewcommand{\@childDeptNameEng}{School of Digital Humanities and Computational Social Sciences}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Digital Humanities and Computational Social Sciences}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{GCT}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{문화기술대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Culture Technology}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Culture Technology}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{STP}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{과학기술정책대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Science and Technology Policy}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Science and Technology Policy}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{GFS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{문술미래전략대학원}
        \renewcommand{\@childDeptNameEng}{Moon Soul Graduate School of Future Strategy}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Future Strategy}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{IP}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{지식재산대학원프로그램}
        \renewcommand{\@childDeptNameEng}{Master’s Program in Intellectual Property}
        \renewcommand{\@parentDeptNameKor}{문술미래전략대학원}
        \renewcommand{\@parentDeptNameEng}{Moon Soul Graduate School of Future Strategy}
        \renewcommand{\@parentAcademNameEng}{Future Strategy}
        \renewcommand{\@childAcademNameEng}{Intellectual Property}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{SJ}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{과학저널리즘대학원프로그램}
        \renewcommand{\@childDeptNameEng}{Master’s Program in Science Journalism}
        \renewcommand{\@parentDeptNameKor}{문술미래전략대학원}
        \renewcommand{\@parentDeptNameEng}{Moon Soul Graduate School of Future Strategy}
        \renewcommand{\@parentAcademNameEng}{Future Strategy}
        \renewcommand{\@childAcademNameEng}{Science Journalism}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{FS}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{미래전략대학원프로그램}
        \renewcommand{\@childDeptNameEng}{Master’s Program in Future Strategy}
        \renewcommand{\@parentDeptNameKor}{문술미래전략대학원}
        \renewcommand{\@parentDeptNameEng}{Moon Soul Graduate School of Future Strategy}
        \renewcommand{\@parentAcademNameEng}{Future Strategy}
        \renewcommand{\@childAcademNameEng}{Future Strategy}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{BTM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{기술경영학부}
        \renewcommand{\@childDeptNameEng}{School of Business and Technology Management}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Business and Technology Management}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{IT}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{기술경영학부 (IT경영학)}
        \renewcommand{\@childDeptNameEng}{School of Business and Technology Management (IT Business)}
        \renewcommand{\@parentDeptNameKor}{기술경영학부}
        \renewcommand{\@parentDeptNameEng}{School of Business and Technology Management}
        \renewcommand{\@parentAcademNameEng}{Business and Technology Management}
        \renewcommand{\@childAcademNameEng}{IT Business}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{GDI}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{글로벌디지털혁신대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Global Digital Innovation}
        \renewcommand{\@parentDeptNameKor}{기술경영학부}
        \renewcommand{\@parentDeptNameEng}{School of Business and Technology Management}
        \renewcommand{\@parentAcademNameEng}{Business and Technology Management}
        \renewcommand{\@childAcademNameEng}{Global Digital Innovation}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{ITM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{기술경영전문대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Innovation and Technology Management}
        \renewcommand{\@parentDeptNameKor}{기술경영학부}
        \renewcommand{\@parentDeptNameEng}{School of Business and Technology Management}
        \renewcommand{\@parentAcademNameEng}{Business and Technology Management}
        \renewcommand{\@childAcademNameEng}{Innovation and Technology Management}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{BIM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{바이오혁신경영전문대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Bio Innovation Management}
        \renewcommand{\@parentDeptNameKor}{기술경영학부}
        \renewcommand{\@parentDeptNameEng}{School of Business and Technology Management}
        \renewcommand{\@parentAcademNameEng}{Business and Technology Management}
        \renewcommand{\@childAcademNameEng}{Bio Innovation Management}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{MT}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{경영공학부}
        \renewcommand{\@childDeptNameEng}{School of Management Engineering}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Management Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{FIN}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{금융MBA}
        \renewcommand{\@childDeptNameEng}{Finance MBA}
        \renewcommand{\@parentDeptNameKor}{금융전문대학원}
        \renewcommand{\@parentDeptNameEng}{Graduate School of Finance}
        \renewcommand{\@parentAcademNameEng}{Finance}
        \renewcommand{\@childAcademNameEng}{Finance MBA}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{FE}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{금융공학프로그램}
        \renewcommand{\@childDeptNameEng}{Financial Engineering Program}
        \renewcommand{\@parentDeptNameKor}{금융전문대학원}
        \renewcommand{\@parentDeptNameEng}{Graduate School of Finance}
        \renewcommand{\@parentAcademNameEng}{Finance}
        \renewcommand{\@childAcademNameEng}{Financial Engineering}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{DF}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{디지털금융MBA}
        \renewcommand{\@childDeptNameEng}{Digital Finance MBA}
        \renewcommand{\@parentDeptNameKor}{금융전문대학원}
        \renewcommand{\@parentDeptNameEng}{Graduate School of Finance}
        \renewcommand{\@parentAcademNameEng}{Finance}
        \renewcommand{\@childAcademNameEng}{Digital Finance MBA}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{FEM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{금융이그제큐티브MBA}
        \renewcommand{\@childDeptNameEng}{Finance Executive MBA}
        \renewcommand{\@parentDeptNameKor}{금융전문대학원}
        \renewcommand{\@parentDeptNameEng}{Graduate School of Finance}
        \renewcommand{\@parentAcademNameEng}{Finance}
        \renewcommand{\@childAcademNameEng}{Finance Executive MBA}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{EM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{이그제큐티브MBA}
        \renewcommand{\@childDeptNameEng}{Executive MBA}
        \renewcommand{\@parentDeptNameKor}{KAIST경영전문대학원}
        \renewcommand{\@parentDeptNameEng}{KAIST Graduate School of Business}
        \renewcommand{\@parentAcademNameEng}{Business}
        \renewcommand{\@childAcademNameEng}{Executive MBA}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{PM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{프로페셔널MBA}
        \renewcommand{\@childDeptNameEng}{Professional MBA}
        \renewcommand{\@parentDeptNameKor}{KAIST경영전문대학원}
        \renewcommand{\@parentDeptNameEng}{KAIST Graduate School of Business}
        \renewcommand{\@parentAcademNameEng}{Business}
        \renewcommand{\@childAcademNameEng}{Professional MBA}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{TM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{테크노경영MBA}
        \renewcommand{\@childDeptNameEng}{Techno-MBA}
        \renewcommand{\@parentDeptNameKor}{KAIST경영전문대학원}
        \renewcommand{\@parentDeptNameEng}{KAIST Graduate School of Business}
        \renewcommand{\@parentAcademNameEng}{Business}
        \renewcommand{\@childAcademNameEng}{Techno-MBA}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{SM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{사회적기업가MBA}
        \renewcommand{\@childDeptNameEng}{Social Entrepreneurship MBA }
        \renewcommand{\@parentDeptNameKor}{KAIST경영전문대학원}
        \renewcommand{\@parentDeptNameEng}{KAIST Graduate School of Business}
        \renewcommand{\@parentAcademNameEng}{Business}
        \renewcommand{\@childAcademNameEng}{Social Entrepreneurship MBA}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{IMM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{정보미디어MBA}
        \renewcommand{\@childDeptNameEng}{Information and Media MBA}
        \renewcommand{\@parentDeptNameKor}{KAIST경영전문대학원}
        \renewcommand{\@parentDeptNameEng}{KAIST Graduate School of Business}
        \renewcommand{\@parentAcademNameEng}{Business}
        \renewcommand{\@childAcademNameEng}{Information and Media MBA}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{IM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{정보경영프로그램}
        \renewcommand{\@childDeptNameEng}{Information Management Program}
        \renewcommand{\@parentDeptNameKor}{KAIST경영전문대학원}
        \renewcommand{\@parentDeptNameEng}{KAIST Graduate School of Business}
        \renewcommand{\@parentAcademNameEng}{Business}
        \renewcommand{\@childAcademNameEng}{Information Management}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{GBP}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{녹색경영정책프로그램}
        \renewcommand{\@childDeptNameEng}{Green Business and Policy Program}
        \renewcommand{\@parentDeptNameKor}{KAIST경영전문대학원}
        \renewcommand{\@parentDeptNameEng}{KAIST Graduate School of Business}
        \renewcommand{\@parentAcademNameEng}{Business}
        \renewcommand{\@childAcademNameEng}{Green Business and Policy}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{KM}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{카이스트MBA}
        \renewcommand{\@childDeptNameEng}{KAIST MBA}
        \renewcommand{\@parentDeptNameKor}{KAIST경영전문대학원}
        \renewcommand{\@parentDeptNameEng}{KAIST Graduate School of Business}
        \renewcommand{\@parentAcademNameEng}{Business}
        \renewcommand{\@childAcademNameEng}{KAIST MBA}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{IMP}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{임팩트MBA}
        \renewcommand{\@childDeptNameEng}{Impact MBA}
        \renewcommand{\@parentDeptNameKor}{KAIST경영전문대학원}
        \renewcommand{\@parentDeptNameEng}{KAIST Graduate School of Business}
        \renewcommand{\@parentAcademNameEng}{Business}
        \renewcommand{\@childAcademNameEng}{Impact MBA}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}
    \ifthenelse{\equal{#1}{SST}}
        {\renewcommand{\@degreeCode}{\@degreePrefix #1}
        \renewcommand{\@childDeptNameKor}{안보과학기술대학원}
        \renewcommand{\@childDeptNameEng}{Graduate School of Advanced Security Science and Technology}
        \renewcommand{\@parentDeptNameKor}{}
        \renewcommand{\@parentDeptNameEng}{}
        \renewcommand{\@parentAcademNameEng}{}
        \renewcommand{\@childAcademNameEng}{Advanced Security Science and Technology}
        \renewcommand{\@degreeField}{#2}
        \renewcommand{\@degreeversion}{#3}}{}

    \renewcommand{\@affFullNameKor}{% 학과/전공 한글이름
        \ifthenelse{\equal{\@parentDeptNameKor}{}}
        {\@childDeptNameKor}{%
            \ifthenelse{\equal{\@degreeversion}{a}}{\@parentDeptNameKor}{}%
            \ifthenelse{\equal{\@degreeversion}{b}}{\@parentDeptNameKor \ (\@childDeptNameKor)}{}%
            \ifthenelse{\equal{\@degreeversion}{c}}{\@childDeptNameKor}{}}
    }
    \renewcommand{\@affFullNameEng}{% 학과/전공 영문이름
        \ifthenelse{\equal{\@parentDeptNameEng}{}}
        {\@childDeptNameEng}{%
            \ifthenelse{\equal{\@degreeversion}{a}}{\@parentDeptNameEng}{}%
            \ifthenelse{\equal{\@degreeversion}{b}}{\@parentDeptNameEng \ (\@childDeptNameEng)}{}%
            \ifthenelse{\equal{\@degreeversion}{c}}{\@childDeptNameEng}{}}
    }
    \renewcommand{\@appFullAcademName}{% 학문 승인서용 영문이름
        \ifthenelse{\equal{\@parentAcademNameEng}{}}
        {\@childAcademNameEng}{%
            \ifthenelse{\equal{\@degreeversion}{a}}{\@parentAcademNameEng}{}%
            \ifthenelse{\equal{\@degreeversion}{b}}{\@parentAcademNameEng \ (\@childAcademNameEng)}{}%
            \ifthenelse{\equal{\@degreeversion}{c}}{\@childAcademNameEng}{}}
    }
    \renewcommand{\@degreeName}{% 학위 영문이름
        \ifthenelse{\boolean{@isDoctor}}
        {Doctor of Philosophy} {% 박사는 모두 Ph.D.
            \ifthenelse{\equal{\@degreeField}{science}}
            {Master of Science}{}% 이학석사는 M.S.
            \ifthenelse{\equal{\@degreeField}{engineering}}
            {Master of Science}{}% 공학석사는 M.S.
            \ifthenelse{\equal{\@degreeField}{business}}
            {Master of Business Administration}{}% 경영학석사는 M.B.A.
        }
    }
}
\@onlypreamble{\department}
